A Preconditioned Discontinuous Galerkin Method for Biharmonic Equation with $C^0$-Reconstructed Approximation

In this paper, we present a high-order finite element method based on a reconstructed approximation to the biharmonic equation. In our construction, the space is reconstructed from nodal values by solving a local least squares fitting problem per element. It is shown that the space can achieve an arbitrarily high-order accuracy and share the same nodal degrees of freedom with the $C^0$ linear space. The interior penalty discontinuous Galerkin scheme can be directly applied to the reconstructed space for solving the biharmonic equation. We prove that the numerical solution converges with optimal orders under error measurements. More importantly, we establish a norm equivalence between the reconstructed space and the continuous linear space. This property allows us to precondition the linear system arising from the high-order space by the linear space on the same mesh. This preconditioner is shown to be optimal in the sense that the condition number of the preconditioned system admits a uniform upper bound independent of the mesh size. Numerical examples in two and three dimensions are provided to illustrate the accuracy of the scheme and the efficiency of the preconditioning method.

==> figure/S0K.tex <==
\fill[blue] (0.516322,0.445641 ) -- ( 0.679732,0.569135 ) -- ( 0.508059,0.641022 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0,0 );
\draw[thick, black] ( 0,0 ) -- ( 0.2,0 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0,0 );
\draw[thick, black] ( 0,0 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.2,0 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.2,0 );
\draw[thick, black] ( 0,0.4 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0,0.4 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0,0.4 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0,0.4 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0,0.6 ) -- ( 0,0.4 );
\draw[thick, black] ( 0,0.4 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0,0.6 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0,0.6 );
\draw[thick, black] ( 0,0.6 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0,0.8 ) -- ( 0,0.6 );
\draw[thick, black] ( 0,0.6 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0,0.8 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0,0.8 );
\draw[thick, black] ( 0,0.8 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 1,0 );
\draw[thick, black] ( 1,0 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0,1 );
\draw[thick, black] ( 0,1 ) -- ( 0,0.8 );
\draw[thick, black] ( 0,0.8 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 1,0.2 );
\draw[thick, black] ( 1,0.2 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 1,0 );
\draw[thick, black] ( 1,0 ) -- ( 1,0.2 );
\draw[thick, black] ( 1,0.2 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0,1 );
\draw[thick, black] ( 0,1 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 1,0.2 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 1,0.2 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 1,1 );
\draw[thick, black] ( 1,1 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 1,1 );
\draw[thick, black] ( 1,1 ) -- ( 0.864919,0.856333 );
\draw[fill = red, red]  (0.129566,0.13237) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0.2,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.2) circle [radius = 0.0085];
\draw[fill = red, red]  (0.289249,0.166948) circle [radius = 0.0085];
\draw[fill = red, red]  (0.158829,0.295084) circle [radius = 0.0085];
\draw[fill = red, red]  (0.4,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.4) circle [radius = 0.0085];
\draw[fill = red, red]  (0.340392,0.360085) circle [radius = 0.0085];
\draw[fill = red, red]  (0.507386,0.214426) circle [radius = 0.0085];
\draw[fill = red, red]  (0.194389,0.511473) circle [radius = 0.0085];
\draw[fill = red, red]  (0.6,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.6) circle [radius = 0.0085];
\draw[fill = red, red]  (0.516322,0.445641) circle [radius = 0.0085];
\draw[fill = red, red]  (0.377541,0.527424) circle [radius = 0.0085];
\draw[fill = red, red]  (0.720368,0.166465) circle [radius = 0.0085];
\draw[fill = red, red]  (0.155049,0.719006) circle [radius = 0.0085];
\draw[fill = red, red]  (0.686727,0.361868) circle [radius = 0.0085];
\draw[fill = red, red]  (0.329937,0.679348) circle [radius = 0.0085];
\draw[fill = red, red]  (0.8,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0.508059,0.641022) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.8) circle [radius = 0.0085];
\draw[fill = red, red]  (0.679732,0.569135) circle [radius = 0.0085];
\draw[fill = red, red]  (0.854173,0.290767) circle [radius = 0.0085];
\draw[fill = red, red]  (0.279589,0.849922) circle [radius = 0.0085];
\draw[fill = red, red]  (0.874828,0.131478) circle [radius = 0.0085];
\draw[fill = red, red]  (0.126891,0.873742) circle [radius = 0.0085];
\draw[fill = red, red]  (0.466174,0.827842) circle [radius = 0.0085];
\draw[fill = red, red]  (0.844029,0.484446) circle [radius = 0.0085];
\draw[fill = red, red]  (0.680339,0.796998) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.2) circle [radius = 0.0085];
\draw[fill = red, red]  (0.844679,0.684532) circle [radius = 0.0085];
\draw[fill = red, red]  (0.2,1) circle [radius = 0.0085];
\draw[fill = red, red]  (0.4,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.4) circle [radius = 0.0085];
\draw[fill = red, red]  (0.6,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.6) circle [radius = 0.0085];
\draw[fill = red, red]  (0.864919,0.856333) circle [radius = 0.0085];
\draw[fill = red, red]  (0.8,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.8) circle [radius = 0.0085];
\draw[fill = red, red]  (1,1) circle [radius = 0.0085];


==> figure/S1K.tex <==
\fill[blue!50] (0.377541,0.527424 ) -- ( 0.516322,0.445641 ) -- ( 0.508059,0.641022 ) -- ( 0.377541,0.527424 );
\fill[blue!50] (0.516322,0.445641 ) -- ( 0.686727,0.361868 ) -- ( 0.679732,0.569135 ) -- ( 0.516322,0.445641 );
\fill[blue!50] (0.680339,0.796998 ) -- ( 0.508059,0.641022 ) -- ( 0.679732,0.569135 ) -- ( 0.680339,0.796998 );
\fill[blue] (0.516322,0.445641 ) -- ( 0.679732,0.569135 ) -- ( 0.508059,0.641022 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0,0 );
\draw[thick, black] ( 0,0 ) -- ( 0.2,0 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0,0 );
\draw[thick, black] ( 0,0 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.2,0 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.2,0 );
\draw[thick, black] ( 0,0.4 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0,0.4 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0,0.4 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0,0.4 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0,0.6 ) -- ( 0,0.4 );
\draw[thick, black] ( 0,0.4 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0,0.6 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0,0.6 );
\draw[thick, black] ( 0,0.6 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0,0.8 ) -- ( 0,0.6 );
\draw[thick, black] ( 0,0.6 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0,0.8 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0,0.8 );
\draw[thick, black] ( 0,0.8 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 1,0 );
\draw[thick, black] ( 1,0 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0,1 );
\draw[thick, black] ( 0,1 ) -- ( 0,0.8 );
\draw[thick, black] ( 0,0.8 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 1,0.2 );
\draw[thick, black] ( 1,0.2 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 1,0 );
\draw[thick, black] ( 1,0 ) -- ( 1,0.2 );
\draw[thick, black] ( 1,0.2 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0,1 );
\draw[thick, black] ( 0,1 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 1,0.2 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 1,0.2 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 1,1 );
\draw[thick, black] ( 1,1 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 1,1 );
\draw[thick, black] ( 1,1 ) -- ( 0.864919,0.856333 );
\draw[fill = red, red]  (0.129566,0.13237) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0.2,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.2) circle [radius = 0.0085];
\draw[fill = red, red]  (0.289249,0.166948) circle [radius = 0.0085];
\draw[fill = red, red]  (0.158829,0.295084) circle [radius = 0.0085];
\draw[fill = red, red]  (0.4,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.4) circle [radius = 0.0085];
\draw[fill = red, red]  (0.340392,0.360085) circle [radius = 0.0085];
\draw[fill = red, red]  (0.507386,0.214426) circle [radius = 0.0085];
\draw[fill = red, red]  (0.194389,0.511473) circle [radius = 0.0085];
\draw[fill = red, red]  (0.6,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.6) circle [radius = 0.0085];
\draw[fill = red, red]  (0.516322,0.445641) circle [radius = 0.0085];
\draw[fill = red, red]  (0.377541,0.527424) circle [radius = 0.0085];
\draw[fill = red, red]  (0.720368,0.166465) circle [radius = 0.0085];
\draw[fill = red, red]  (0.155049,0.719006) circle [radius = 0.0085];
\draw[fill = red, red]  (0.686727,0.361868) circle [radius = 0.0085];
\draw[fill = red, red]  (0.329937,0.679348) circle [radius = 0.0085];
\draw[fill = red, red]  (0.8,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0.508059,0.641022) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.8) circle [radius = 0.0085];
\draw[fill = red, red]  (0.679732,0.569135) circle [radius = 0.0085];
\draw[fill = red, red]  (0.854173,0.290767) circle [radius = 0.0085];
\draw[fill = red, red]  (0.279589,0.849922) circle [radius = 0.0085];
\draw[fill = red, red]  (0.874828,0.131478) circle [radius = 0.0085];
\draw[fill = red, red]  (0.126891,0.873742) circle [radius = 0.0085];
\draw[fill = red, red]  (0.466174,0.827842) circle [radius = 0.0085];
\draw[fill = red, red]  (0.844029,0.484446) circle [radius = 0.0085];
\draw[fill = red, red]  (0.680339,0.796998) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.2) circle [radius = 0.0085];
\draw[fill = red, red]  (0.844679,0.684532) circle [radius = 0.0085];
\draw[fill = red, red]  (0.2,1) circle [radius = 0.0085];
\draw[fill = red, red]  (0.4,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.4) circle [radius = 0.0085];
\draw[fill = red, red]  (0.6,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.6) circle [radius = 0.0085];
\draw[fill = red, red]  (0.864919,0.856333) circle [radius = 0.0085];
\draw[fill = red, red]  (0.8,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.8) circle [radius = 0.0085];
\draw[fill = red, red]  (1,1) circle [radius = 0.0085];


==> figure/S2K.tex <==
\fill[blue!50] (0.377541,0.527424 ) -- ( 0.340392,0.360085 ) -- ( 0.516322,0.445641 ) -- ( 0.377541,0.527424 );
\fill[blue!50] (0.516322,0.445641 ) -- ( 0.507386,0.214426 ) -- ( 0.686727,0.361868 ) -- ( 0.516322,0.445641 );
\fill[blue!50] (0.377541,0.527424 ) -- ( 0.516322,0.445641 ) -- ( 0.508059,0.641022 ) -- ( 0.377541,0.527424 );
\fill[blue!50] (0.508059,0.641022 ) -- ( 0.329937,0.679348 ) -- ( 0.377541,0.527424 ) -- ( 0.508059,0.641022 );
\fill[blue!50] (0.516322,0.445641 ) -- ( 0.686727,0.361868 ) -- ( 0.679732,0.569135 ) -- ( 0.516322,0.445641 );
\fill[blue!50] (0.686727,0.361868 ) -- ( 0.844029,0.484446 ) -- ( 0.679732,0.569135 ) -- ( 0.686727,0.361868 );
\fill[blue!50] (0.680339,0.796998 ) -- ( 0.508059,0.641022 ) -- ( 0.679732,0.569135 ) -- ( 0.680339,0.796998 );
\fill[blue!50] (0.680339,0.796998 ) -- ( 0.466174,0.827842 ) -- ( 0.508059,0.641022 ) -- ( 0.680339,0.796998 );
\fill[blue!50] (0.679732,0.569135 ) -- ( 0.844679,0.684532 ) -- ( 0.680339,0.796998 ) -- ( 0.679732,0.569135 );
\fill[blue] (0.516322,0.445641 ) -- ( 0.679732,0.569135 ) -- ( 0.508059,0.641022 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0,0 );
\draw[thick, black] ( 0,0 ) -- ( 0.2,0 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0,0 );
\draw[thick, black] ( 0,0 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.2,0 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.2,0 );
\draw[thick, black] ( 0,0.4 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0,0.4 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0,0.4 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0,0.4 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0,0.6 ) -- ( 0,0.4 );
\draw[thick, black] ( 0,0.4 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0,0.6 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0,0.6 );
\draw[thick, black] ( 0,0.6 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0,0.8 ) -- ( 0,0.6 );
\draw[thick, black] ( 0,0.6 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0,0.8 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0,0.8 );
\draw[thick, black] ( 0,0.8 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 1,0 );
\draw[thick, black] ( 1,0 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0,1 );
\draw[thick, black] ( 0,1 ) -- ( 0,0.8 );
\draw[thick, black] ( 0,0.8 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 1,0.2 );
\draw[thick, black] ( 1,0.2 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 1,0 );
\draw[thick, black] ( 1,0 ) -- ( 1,0.2 );
\draw[thick, black] ( 1,0.2 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0,1 );
\draw[thick, black] ( 0,1 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 1,0.2 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 1,0.2 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 1,1 );
\draw[thick, black] ( 1,1 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 1,1 );
\draw[thick, black] ( 1,1 ) -- ( 0.864919,0.856333 );
\draw[fill = red, red]  (0.129566,0.13237) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0.2,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.2) circle [radius = 0.0085];
\draw[fill = red, red]  (0.289249,0.166948) circle [radius = 0.0085];
\draw[fill = red, red]  (0.158829,0.295084) circle [radius = 0.0085];
\draw[fill = red, red]  (0.4,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.4) circle [radius = 0.0085];
\draw[fill = red, red]  (0.340392,0.360085) circle [radius = 0.0085];
\draw[fill = red, red]  (0.507386,0.214426) circle [radius = 0.0085];
\draw[fill = red, red]  (0.194389,0.511473) circle [radius = 0.0085];
\draw[fill = red, red]  (0.6,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.6) circle [radius = 0.0085];
\draw[fill = red, red]  (0.516322,0.445641) circle [radius = 0.0085];
\draw[fill = red, red]  (0.377541,0.527424) circle [radius = 0.0085];
\draw[fill = red, red]  (0.720368,0.166465) circle [radius = 0.0085];
\draw[fill = red, red]  (0.155049,0.719006) circle [radius = 0.0085];
\draw[fill = red, red]  (0.686727,0.361868) circle [radius = 0.0085];
\draw[fill = red, red]  (0.329937,0.679348) circle [radius = 0.0085];
\draw[fill = red, red]  (0.8,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0.508059,0.641022) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.8) circle [radius = 0.0085];
\draw[fill = red, red]  (0.679732,0.569135) circle [radius = 0.0085];
\draw[fill = red, red]  (0.854173,0.290767) circle [radius = 0.0085];
\draw[fill = red, red]  (0.279589,0.849922) circle [radius = 0.0085];
\draw[fill = red, red]  (0.874828,0.131478) circle [radius = 0.0085];
\draw[fill = red, red]  (0.126891,0.873742) circle [radius = 0.0085];
\draw[fill = red, red]  (0.466174,0.827842) circle [radius = 0.0085];
\draw[fill = red, red]  (0.844029,0.484446) circle [radius = 0.0085];
\draw[fill = red, red]  (0.680339,0.796998) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.2) circle [radius = 0.0085];
\draw[fill = red, red]  (0.844679,0.684532) circle [radius = 0.0085];
\draw[fill = red, red]  (0.2,1) circle [radius = 0.0085];
\draw[fill = red, red]  (0.4,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.4) circle [radius = 0.0085];
\draw[fill = red, red]  (0.6,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.6) circle [radius = 0.0085];
\draw[fill = red, red]  (0.864919,0.856333) circle [radius = 0.0085];
\draw[fill = red, red]  (0.8,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.8) circle [radius = 0.0085];
\draw[fill = red, red]  (1,1) circle [radius = 0.0085];


==> figure/S3K.tex <==
\fill[blue!50] (0.377541,0.527424 ) -- ( 0.340392,0.360085 ) -- ( 0.516322,0.445641 ) -- ( 0.377541,0.527424 );
\fill[blue!50] (0.377541,0.527424 ) -- ( 0.516322,0.445641 ) -- ( 0.508059,0.641022 ) -- ( 0.377541,0.527424 );
\fill[blue!50] (0.508059,0.641022 ) -- ( 0.329937,0.679348 ) -- ( 0.377541,0.527424 ) -- ( 0.508059,0.641022 );
\fill[blue!50] (0.516322,0.445641 ) -- ( 0.686727,0.361868 ) -- ( 0.679732,0.569135 ) -- ( 0.516322,0.445641 );
\fill[blue!50] (0.466174,0.827842 ) -- ( 0.329937,0.679348 ) -- ( 0.508059,0.641022 ) -- ( 0.466174,0.827842 );
\fill[blue!50] (0.686727,0.361868 ) -- ( 0.844029,0.484446 ) -- ( 0.679732,0.569135 ) -- ( 0.686727,0.361868 );
\fill[blue!50] (0.680339,0.796998 ) -- ( 0.508059,0.641022 ) -- ( 0.679732,0.569135 ) -- ( 0.680339,0.796998 );
\fill[blue!50] (0.680339,0.796998 ) -- ( 0.466174,0.827842 ) -- ( 0.508059,0.641022 ) -- ( 0.680339,0.796998 );
\fill[blue] (0.516322,0.445641 ) -- ( 0.679732,0.569135 ) -- ( 0.508059,0.641022 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0,0 );
\draw[thick, black] ( 0,0 ) -- ( 0.2,0 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0,0 );
\draw[thick, black] ( 0,0 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.2,0 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.129566,0.13237 );
\draw[thick, black] ( 0.129566,0.13237 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.2,0 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.2,0 );
\draw[thick, black] ( 0,0.4 ) -- ( 0,0.2 );
\draw[thick, black] ( 0,0.2 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0,0.4 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0.289249,0.166948 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.289249,0.166948 );
\draw[thick, black] ( 0,0.4 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0,0.4 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.158829,0.295084 );
\draw[thick, black] ( 0.158829,0.295084 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.4,0 );
\draw[thick, black] ( 0.4,0 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0,0.6 ) -- ( 0,0.4 );
\draw[thick, black] ( 0,0.4 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0,0.6 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.340392,0.360085 );
\draw[thick, black] ( 0.340392,0.360085 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0,0.6 );
\draw[thick, black] ( 0,0.6 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.507386,0.214426 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.507386,0.214426 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.194389,0.511473 );
\draw[thick, black] ( 0.194389,0.511473 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.6,0 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.6,0 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0,0.8 ) -- ( 0,0.6 );
\draw[thick, black] ( 0,0.6 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0,0.8 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.377541,0.527424 );
\draw[thick, black] ( 0.377541,0.527424 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.516322,0.445641 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.516322,0.445641 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.720368,0.166465 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.720368,0.166465 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0,0.8 );
\draw[thick, black] ( 0,0.8 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.155049,0.719006 );
\draw[thick, black] ( 0.155049,0.719006 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.686727,0.361868 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.686727,0.361868 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.329937,0.679348 );
\draw[thick, black] ( 0.329937,0.679348 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 0.8,0 );
\draw[thick, black] ( 0.8,0 ) -- ( 1,0 );
\draw[thick, black] ( 1,0 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.508059,0.641022 );
\draw[thick, black] ( 0.508059,0.641022 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0,1 );
\draw[thick, black] ( 0,1 ) -- ( 0,0.8 );
\draw[thick, black] ( 0,0.8 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 1,0.2 );
\draw[thick, black] ( 1,0.2 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.679732,0.569135 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.679732,0.569135 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.874828,0.131478 ) -- ( 1,0 );
\draw[thick, black] ( 1,0 ) -- ( 1,0.2 );
\draw[thick, black] ( 1,0.2 ) -- ( 0.874828,0.131478 );
\draw[thick, black] ( 0.126891,0.873742 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0,1 );
\draw[thick, black] ( 0,1 ) -- ( 0.126891,0.873742 );
\draw[thick, black] ( 1,0.2 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 0.854173,0.290767 );
\draw[thick, black] ( 0.854173,0.290767 ) -- ( 1,0.2 );
\draw[thick, black] ( 0.279589,0.849922 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.2,1 );
\draw[thick, black] ( 0.2,1 ) -- ( 0.279589,0.849922 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.466174,0.827842 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.4,1 );
\draw[thick, black] ( 0.4,1 ) -- ( 0.466174,0.827842 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844029,0.484446 ) -- ( 1,0.4 );
\draw[thick, black] ( 1,0.4 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 0.844029,0.484446 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.6,1 );
\draw[thick, black] ( 0.6,1 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.680339,0.796998 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.680339,0.796998 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 1,0.6 );
\draw[thick, black] ( 1,0.6 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.844679,0.684532 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 0.844679,0.684532 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 1,1 );
\draw[thick, black] ( 1,1 ) -- ( 0.8,1 );
\draw[thick, black] ( 0.8,1 ) -- ( 0.864919,0.856333 );
\draw[thick, black] ( 0.864919,0.856333 ) -- ( 1,0.8 );
\draw[thick, black] ( 1,0.8 ) -- ( 1,1 );
\draw[thick, black] ( 1,1 ) -- ( 0.864919,0.856333 );
\draw[fill = red, red]  (0.129566,0.13237) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0.2,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.2) circle [radius = 0.0085];
\draw[fill = red, red]  (0.289249,0.166948) circle [radius = 0.0085];
\draw[fill = red, red]  (0.158829,0.295084) circle [radius = 0.0085];
\draw[fill = red, red]  (0.4,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.4) circle [radius = 0.0085];
\draw[fill = red, red]  (0.340392,0.360085) circle [radius = 0.0085];
\draw[fill = red, red]  (0.507386,0.214426) circle [radius = 0.0085];
\draw[fill = red, red]  (0.194389,0.511473) circle [radius = 0.0085];
\draw[fill = red, red]  (0.6,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.6) circle [radius = 0.0085];
\draw[fill = red, red]  (0.516322,0.445641) circle [radius = 0.0085];
\draw[fill = red, red]  (0.377541,0.527424) circle [radius = 0.0085];
\draw[fill = red, red]  (0.720368,0.166465) circle [radius = 0.0085];
\draw[fill = red, red]  (0.155049,0.719006) circle [radius = 0.0085];
\draw[fill = red, red]  (0.686727,0.361868) circle [radius = 0.0085];
\draw[fill = red, red]  (0.329937,0.679348) circle [radius = 0.0085];
\draw[fill = red, red]  (0.8,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0.508059,0.641022) circle [radius = 0.0085];
\draw[fill = red, red]  (0,0.8) circle [radius = 0.0085];
\draw[fill = red, red]  (0.679732,0.569135) circle [radius = 0.0085];
\draw[fill = red, red]  (0.854173,0.290767) circle [radius = 0.0085];
\draw[fill = red, red]  (0.279589,0.849922) circle [radius = 0.0085];
\draw[fill = red, red]  (0.874828,0.131478) circle [radius = 0.0085];
\draw[fill = red, red]  (0.126891,0.873742) circle [radius = 0.0085];
\draw[fill = red, red]  (0.466174,0.827842) circle [radius = 0.0085];
\draw[fill = red, red]  (0.844029,0.484446) circle [radius = 0.0085];
\draw[fill = red, red]  (0.680339,0.796998) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0) circle [radius = 0.0085];
\draw[fill = red, red]  (0,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.2) circle [radius = 0.0085];
\draw[fill = red, red]  (0.844679,0.684532) circle [radius = 0.0085];
\draw[fill = red, red]  (0.2,1) circle [radius = 0.0085];
\draw[fill = red, red]  (0.4,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.4) circle [radius = 0.0085];
\draw[fill = red, red]  (0.6,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.6) circle [radius = 0.0085];
\draw[fill = red, red]  (0.864919,0.856333) circle [radius = 0.0085];
\draw[fill = red, red]  (0.8,1) circle [radius = 0.0085];
\draw[fill = red, red]  (1,0.8) circle [radius = 0.0085];
\draw[fill = red, red]  (1,1) circle [radius = 0.0085];

